Metal Price Spike Prediction via a Neurosymbolic Ensemble Approach

Predicting price spikes in critical metals such as Cobalt, Copper, Magnesium, and Nickel is crucial for mitigating economic risks associated with global trends like the energy transition and reshoring of manufacturing. While traditional models have focused on regression-based approaches, our work introduces a neurosymbolic ensemble framework that integrates multiple neural models with symbolic error detection and correction rules. This framework is designed to enhance predictive accuracy by correcting individual model errors and offering interpretability through rule-based explanations. We show that our method provides up to 6.42% improvement in precision, 29.41% increase in recall at 13.24% increase in F1 over the best performing neural models. Further, our method, as it is based on logical rules, has the benefit of affording an explanation as to which combination of neural models directly contribute to a given prediction.

==> diagrams/graphs.tex <==
\begin{figure}[hbt!]
    \centering
    \includegraphics[width=0.8\textwidth]{diagrams/pre-rec_graphs/pr.png}
    \caption{Performance of the LSTM (1) model (left) and CNN Attention (5) model in predicting Cobalt and Nickel price spikes respectively. The x-axis represents threshold values of Training F1 scores that determine the ruleset inclusion.}
    \label{fig:graph1}
\end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\textwidth]{diagrams/ablation_charts/cop8.png}
%     \caption{Ablation analysis of EDCR on CNN model performance metrics for predicting Copper price spikes. The bar charts reveal that removing CNN, RNN, and CNN Attention from the ruleset results in a significant drop in both Precision and Recall. Conversely, the removal of LSTM has no impact on performance, indicating its redundancy in this specific ruleset configuration.}
%     \label{fig:ablation1}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{diagrams/ablation2.png}
%     \caption{Ablation analysis of EDCR on model performance metrics. In cases where EDCR has no effect on base model performance, the ablation study shows that removing models from the ruleset will have no effect as well.}
%     \label{fig:ablation2}
% \end{figure}
